Spectral band selection for vegetation properties retrieval using Gaussian processes regression

With current and upcoming imaging spectrometers, automated band analysis techniques are needed to enable efficient identification of most informative bands to facilitate optimized processing of spectral data into estimates of biophysical variables. This paper introduces an automated spectral band analysis tool (BAT) based on Gaussian processes regression (GPR) for the spectral analysis of vegetation properties. The GPR-BAT procedure sequentially backwards removes the least contributing band in the regression model for a given variable until only one band is kept. GPR-BAT is implemented within the framework of the free ARTMO's MLRA (machine learning regression algorithms) toolbox, which is dedicated to the transforming of optical remote sensing images into biophysical products. GPR-BAT allows (1) to identify the most informative bands in relating spectral data to a biophysical variable, and (2) to find the least number of bands that preserve optimized accurate predictions. This study concludes that a wise band selection of hyperspectral data is strictly required for optimal vegetation properties mapping.

==> GPR_theory.tex <==
Estimation, regression and function approximation are old, largely studied problems in statistics and machine learning. The problem boils down to optimize a loss (cost, energy) function over a class of functions. A large class of regression problems in particular are defined as the joint minimization of a loss function accounting for errors of the function $f\in {\mathcal H}$ to be learned, and a regularization term, $\Omega\left(\|f\|^2_{{\mathcal H}}\right)$, that controls its capacity (excess of flexibility). The problem can be approached within a Bayesian nonparametric framework, and several algorithms are available, such as the relevance vector machine~\citep{Tipping2001a,campsvalls06rvm} or Gaussian Processes regression (GPR)~\citep{Rasmussen06,CampsValls16grsm}, in which we will focus here. 


GPR is equivalent in nature to kernel ridge regression (aka least square support vector machine) and kriging. However, due to their high computational complexity they did not become widely applied tools in machine learning until recently.
GPR can be interpreted as a family of kernel methods with the additional advantage of providing a full conditional statistical description for the predicted variable, which can be primarily used to establish confidence intervals and to set hyper-parameters \citep{Rasmussen06}. In short, GPR assumes that a Gaussian process prior governs the set of possible latent functions (which are unobserved), and the likelihood (of the latent function) and observations shape this prior to produce posterior probabilistic estimates. Consequently, the joint distribution of training and test data is a multidimensional Gaussian and the predicted distribution is estimated by conditioning on the training data. 

Standard regression approximates observations (often referred to as \emph{outputs}) $\{y_n\}_{n=1}^{N}$  as the sum of some unknown latent function $f(\x)$ of the $N$ input points $\x_n = [x_n^1,\ldots,x_n^B]$ (spectra) of dimensionality $B$ (bands) plus Gaussian noise, i.e. 
\begin{equation}\label{GLR}
y_n = f(\x_n) + \varepsilon_n,~~~\varepsilon_n \sim\Normal(0,\sigma^2).
\end{equation}
Instead of proposing a parametric form for $f(\x)$ and learning its parameters in order to fit observed data well,  GP regression proceeds in a Bayesian, non-parametric way. A zero mean\footnote{It is customary to subtract the sample mean to data $\{y_n\}_{n=1}^N$, and then to assume a zero mean model.} GP prior is placed on the latent function $f({\bf x})$ and a Gaussian prior is used for each latent noise term $\varepsilon_n$, 
$f({\bf x})\;\sim\;\GP({\bf 0}, k_{\bf \theta}({\bf x},{\bf x}'))$, 
where $k_{\bf \theta}({\bf x},{\bf x}')$ is a covariance function parametrized by ${\bf \theta}$ and $\sigma^2$ is a hyperparameter that specifies the noise power.
Essentially, a GP is a stochastic process whose marginals are distributed as a multivariate Gaussian. In particular, given the priors $\GP$, samples drawn from $f(\x)$ at the set of locations $\{\x_n\}_{n=1}^N$ follow a joint multivariate Gaussian with zero mean and covariance matrix $\Kbf_{\bf ff}$ with  $[\Kbf_{\bf ff}]_{ij} = k_{\bf \theta}({\bf x}_i,{\bf x}_j)$.

If we consider a test location $\x_*$ with corresponding output $y_*$, priors $\GP$ induce a %the following  joint 
prior distribution between the observations $\y \equiv \{y_n\}_{n=1}^N$ and $y_*$.
Collecting available data in $\dataset\equiv\{{\bf x}_n,y_n|n=1,\ldots
N\}$, it is possible to analytically compute the posterior distribution over the unknown output $y_*$: 
\begin{align}
 \prob(y_*|{\bf x}_*,\dataset)&=\Normal(y_*|\mu_{\text{GP}*},\sigma_{\text{GP}*}^2) \\
\mu_{\text{GP}*} &= {\bf k}_{{\bf f}*}^\top (\Kbf_{{\bf ff}}+\sigma^2{\bf I}_n)^{-1}{\bf 
y} = {\bf k}_{{\bf f}*}^\top\boldsymbol{\alpha} \label{eq:mugp}\\
\sigma_{\text{GP}*}^2 &= \sigma^2+k_{**}-
     {\bf k}_{{\bf f}*}^\top (\Kbf_{{\bf ff}}+\sigma^2{\bf I}_n)^{-1}{\bf k}_{\vect
{f}*}. \label{eq:sigmagp}
\end{align}
which is computable in $\bigO(n^3)$ time (this cost arises from the inversion of the $n\times n$ matrix ($\Kbf_{{\bf ff}}+\sigma^2{\bf I}$), see \citep{Rasmussen06}. %, Ch.~8.
In addition to the computational cost, GPs require large memory since in naive implementations one has to store the training kernel matrix, which amounts to ${\mathcal O}(n^2)$. 

 

The corresponding hyperparameters $\{{\bf \theta},\sigma_n\}$ are typically selected by Type-II Maximum Likelihood, using the marginal likelihood (also called evidence) of the observations, which is also analytical (explicitly conditioning on ${\bf \theta}$ and $\sigma_n$):
\begin{equation}
\log p({\bf y}|{\bf \theta},\sigma_n) =  \log \Normal(\y|{\bf 0}, \Kf + \sigma_n^2{\bf I}).
\label{eq:logevidence}
\end{equation}
When the derivatives of \eqref{eq:logevidence} are also analytical, which is often the case, conjugated gradient ascend is typically used for optimization. Therefore, the whole procedure for learning a GP model only depends on a very small set of hyper-parameters that combats overfitting efficiently. Finally, inference of the hyper-parameters and the weights for doing predictions, $\boldsymbol{\alpha}$, can be performed using this continuous optimization of the evidence.

 

The core of any kernel method in general, and of GPs in particular, is the appropriate definition of the covariance (or kernel) function. A standard, widely used covariance function is the squared exponential, 
$$k({\bf x}_i,{\bf x}_j) = \exp(-\|{\bf x}_i-{\bf x}_j\|^2/(2\sigma^2)),$$
which captures sample similarity well in most of the (unstructured) problems, and only one hyperparameter $\sigma$ needs to be tuned. 

In the context of GPs, kernels with more hyperparameters can be efficiently inferred as we have seen before. This is an  opportunity to exploit assymetries in the feature space by including a parameter per feature, as in the very common anisotropic squared exponential (SE) kernel function:
$$k(\x_i,\x_j) = \nu \exp\bigg(-\sum_{b=1}^B \dfrac{(x_i^b-x_j^b)^2}{2\sigma_b^2}\bigg) + \sigma_n^2\delta_{ij},$$
where $\nu$ is a scaling factor, $\sigma_n$ is the standard deviation of the (estimated) noise, and a $\sigma_b$ is the length-scale per input bands  (features), $b=1,\ldots,B$.  This is a very flexible covariance function that typically suffices to tackle most of the problems, especially for smoothly-varying functions.  
Model parameters ($\nu$, $\sigma_b$) and model weights $\alpha_i$ can be automatically optimized by maximizing the marginal likelihood in the training set. The obtained weights $\alpha_i$  after optimization gives the relevance of each spectrum $\x_i$, while the inverse of $\sigma_b$ represents the relevance of each spectral band $B$. Hence, low values of $\sigma_b$ indicate a higher informative content of this certain band $b$ to the training function $k$. This $\sigma_b$ property shall be further exploited in this paper.

 
Specifically, it is proposed to go beyond the standard analysis of the inferred length-scales for a particular run of a GPR \red{model}. We instead exploit this nice property of the ARD covariance in a wrapper strategy. For this, we adopt a simple and general iterative backward greedy algorithm, in which the impact of the inputs on the prediction error is evaluated in the context or absence of the other predictors. Essentially, at each iteration we remove the least significant band, that with highest $\sigma_b$, and retrain a new GPR model with the remaining bands only. This {\em sequential backward band removal} (SBBR) algorithm is similar to the one often applied in classification using support vector machines, referred to as {\em recursive feature elimination} (RFE). In RFE, the feature with the smallest ranking score is eliminated in order to recursively remove insignificant features. However, RFE is merely interested in determining optimized classification results~\citep[e.g.,][]{Bazi2006,Archibald2007,Pal2010}, while here we aim to move backwards until only one band is left in order to identify most informative bands in linking to a biophysical variable. The SBBR routine is summarized in Algorithm \ref{GPR-BAT}.

\begin{algorithm}[h!]
\caption{Sequential backward band removal (SBBR)}
\label{GPR-BAT}
\begin{algorithmic}[1]
\For{Number of bands $D$}
\State Split spectra-variable dataset into training and validation set
\State Train GPR model
\State Rank $\sigma_b$ obtained during GPR model development
\State Calculate score indicators in the validation set: $R^2$, RMSE, NRMSE
\State Remove band with highest $\sigma_b$ from dataset
\EndFor
\end{algorithmic}
\end{algorithm}


In earlier works~\citep{Verrelst12a,Verrelst2012,Wittenberghe2014} we illustrated the usefulness of the SBBR routine for the identification of the most relevant spectral channels for the retrieval of vegetation variables from hyperspectral data. A rudimentary version of the SBBR routine reached high regression accuracies with a minimal amount of bands, i.e. generated GPR models outperformed the case of using all bands. Moreover, in~\citet{Verrelst12a}, it was demonstrated that the SBBR routine led to higher prediction accuracies compared to systematically analyzing all two-band normalized difference combinations. At the same time, the best performing bands proved to have physical meaning, i.e. they were located in relevant absorption regions. To enable automated identification of best performing bands for any paired spectra-variable dataset, in this work we have integrated and automated the SBBR routine into a user-friendly tool, called GPR-BAT.  

